Resilient Ramp Control for Highways Facing Stochastic Perturbations

Highway capacity is often subject to stochastic perturbations due to the combined effects of weather, traffic mixture, driver behavior, etc. This paper is motivated by the need of a systematic approach to traffic control with performance guarantees in the face of such perturbations. We develop a novel control-theoretic method for designing perturbation-resilient ramp metering. We consider a cell-transmission model with 1) Markovian cell capacities and 2) buffers representing on-ramps and upstream mainline. Using this model, we analyze the stability of on-ramp queues by constructing piecewise Lyapunov functions that consider the nature of nonlinear traffic dynamics. Then, we design ramp controllers that guarantee bounds for throughput and queue sizes. We also formulate the problem of coordinated ramp metering as a bi-level optimization with non-convex inner sub-problems. To address the computational issue in solving this problem, we also consider localized and partially coordinated reformulations. A case study of a 18.1-km highway in Los Angeles, USA indicates a 8.3\% (resp. 9.9\%) reduction of vehicle-hours-traveled obtained by the localized (resp. partially coordinated) control, both outperforming the classical ALINEA and METALINE controllers.

==> Texts/Bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Jin.png}}]{Li Jin} is Assistant Professor (2021--present) at the UM Joint Institute and the School of Electronic Information and Electrical Engineering, Shanghai Jiao Tong University, China. He is also Research Assistant Professor and was Assistant Professor (2018--2020) in the Tandon School of Engineering, New York University, USA. He received his B.Eng. from Shanghai Jiao Tong University in 2011, M.S. from Purdue University in 2012, and Ph.D. from the Massachusetts Institute of Technology in 2018. He was also a Visiting Scholar at the University of Erlangen-Nuremberg in 2016. His research uses ideas from stochastic processes, control, optimization, and machine learning to address key challenges in smart and connected systems. Specific applications include connected and autonomous vehicles, intelligent transportation systems, air traffic control, and smart pipeline transportation.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Tang}}]{Yu Tang} is a PhD candidate at the Department of Civil and Urban Engineering and the C2SMART University Transportation Center in the New York University Tandon School of Engineering. He received his B.Eng. and M.S. in Transportation Engineering from Tongji University. He is interested in using ideas from stochastic processes and dynamic control to design resilient intelligent transportation systems.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Kurzhanskiy}}]{Alexander A. Kurzhanskiy} is Assistant Research Engineer at University of California, Berkeley. He received his M.S. in Applied Mathematics from Lomonosov Moscow State University and his Ph.D. in Electrical Engineering \& Computer Science from Berkeley. From 1998 to 2003 he worked for several Silicon Valley companies. His research interests include dynamical systems estimation and control, application of the set-valued calculus to reachability analysis and estimation, robust convex optimization, transportation systems.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Amin}}]{Saurabh Amin} is Robert N. Noyce Career Development Associate Professor in the Department of Civil and Environmental Engineering and a core faculty member in the Laboratory of Information and Decision Systems (LIDS), Massachusetts Institute of Technology. He received his Ph.D. in Systems Engineering from the University of California, Berkeley in 2011. 
His research focuses on the design of implementation of high confidence network control algorithms for infrastructure systems. He works on robust diagnostics and control problems that involve using networked systems to facilitate the monitoring and control of large-scale critical infrastructures, including transportation, water, and energy distribution systems. He also studies the effects of security attacks and random faults on the survivability of networked systems, and designs incentive-compatible control mechanisms to reduce network risks. He is a recipient of NSF CAREER and Google Faculty Research awards.
\end{IEEEbiography}
